JourneyBench: A Challenging One-Stop Vision-Language Understanding Benchmark of Generated Images

Existing vision-language understanding benchmarks largely consist of images of objects in their usual contexts. As a consequence, recent multimodal large language models can perform well with only a shallow visual understanding by relying on background language biases. Thus, strong performance on these benchmarks does not necessarily correlate with strong visual understanding. In this paper, we release JourneyBench, a comprehensive human-annotated benchmark of generated images designed to assess the model's fine-grained multimodal reasoning abilities across five tasks: complementary multimodal chain of thought, multi-image VQA, imaginary image captioning, VQA with hallucination triggers, and fine-grained retrieval with sample-specific distractors. Unlike existing benchmarks, JourneyBench explicitly requires fine-grained multimodal reasoning in unusual imaginary scenarios where language bias and holistic image gist are insufficient. We benchmark state-of-the-art models on JourneyBench and analyze performance along a number of fine-grained dimensions. Results across all five tasks show that JourneyBench is exceptionally challenging for even the best models, indicating that models' visual reasoning abilities are not as strong as they first appear. We discuss the implications of our findings and propose avenues for further research.

==> figures/captioning-across-categories.tex <==
\begin{figure}[ht!]
    \centering
    \captionsetup{skip=5pt}
    \scalebox{0.3}{
    \includegraphics{figures/captioning-across-categories.pdf}
    }
    % \vspace{-0.5em}
  \caption{.}
  \label{fig:captioning-across-categories}
  % \vspace{-1em}
\end{figure}

==> figures/category_unusalness.tex <==
\begin{figure}[ht!]
    \centering
    \captionsetup{skip=5pt}
    \scalebox{0.3}{
    \includegraphics{figures/category_unusualness.pdf}
    }
    % \vspace{-0.5em}
  \caption{.}
  \label{fig:category_unusualness}
  % \vspace{-1em}
\end{figure}

==> figures/fine-grained_cr_across_categories.tex <==
\begin{figure}[ht!]
    \centering
    \captionsetup{skip=5pt}
    \scalebox{0.4}{
    \includegraphics{figures/fine-grained_cr_across_categories.pdf}
    }
    % \vspace{-0.5em}
  \caption{.}
  \label{fig:fine-grained_cr_across_categories}
  % \vspace{-1em}
\end{figure}

==> figures/pie_chart_query_words.tex <==
\begin{figure}[ht!]
    \centering
    \captionsetup{skip=5pt}
    \scalebox{0.3}{
    \includegraphics{figures/pie_chart_query_words.pdf}
    }
    % \vspace{-0.5em}
  \caption{.}
  \label{fig:pie_chart_query_words}
  % \vspace{-1em}
\end{figure}

==> tables/combine_table.tex <==

\begin{table}[t]
\captionsetup{skip=5pt}
\centering
\fontsize{8}{9}\selectfont
\setlength{\tabcolsep}{3pt}

\begin{minipage}[t]{0.48\textwidth}
    \centering
    \resizebox{72mm}{!}{%
     \begin{tabular}{l|l|l|m{1 cm}|m{1 cm}|c|l}  \hline \hline
\multirow{3}{*}{Model} & \multicolumn{5}{c|}{Multi-Image VQA} & \multirow{3}{*}{\makecell{Mantis\\Eval}} \\ \cline{2-6}
   &   \multirow{2}{*}{All} &  \multicolumn{3}{c|}{MMCOT} & \multirow{2}{*}{\makecell{Cause \\and \\ Effect}} &  \\ \cline{3-5}
   &   & \multicolumn{1}{l|}{All} &\multicolumn{1}{l|}{\makecell{Arithmetic \\ Reasoning}} & \multicolumn{1}{l|}{\makecell{External\\Knowledge}} &   & \\ \hline
VILA-8B~\cite{vila}            &    24.20   & 6.14  & 3.73  & 8.65  & 53.92 & 51.15 \\
Idefics2-8B~\cite{idefics2}        & 27.82 & 6.61  & 2.81  & 10.57 & 65.03 & 48.85 \\
Mantis-Idefics2-8B~\cite{mantis} & 19.90 & 3.30  & 3.71  & 2.88  & 49.02 & 57.14 \\
Mantis-SigLIP-8B~\cite{mantis}   & 23.29 & 4.72  & 5.98  & 3.41  & 55.88 & 59.45 \\
GPT-4V~              & 48.70 & 32.54 & 32.88 & \textbf{32.2}  &77.06 & 62.67 \\
GPT-4o~              & \textbf{56.39} & \textbf{41.03} & \textbf{52.04} & 29.61& \textbf{83.33} &  \textbf{73.42}   \\ \hline \hline
\end{tabular}
}
\caption{\small{\textbf{Zero-shot Evaluation on Multi-Image Reasoning.} The best results are highlighted in bold. Baseline models like GPT-4o perform significantly worse on our Multi-image VQA or MMCOT than on Mantis-Eval. Note that most models on Cause and Effect - being a binary-choice question - have an accuracy of nearly random guessing. }}
\label{tab:multi-image mcot}
\end{minipage}\hfill
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \resizebox{68mm}{!}{%
        \begin{tabular}{l|l|lcl} \hline \hline
        Model                    & BLEU1-4         & CIDEr        & METEOR       & Rouge        \\ \hline
MiniGPT4-LLama2-7B~\cite{minigpt}      & 19.60	& 20.91	&  18.07	&  28.76 \\
mPLUG-Owl-7.2B~\cite{mplug}       & 19.53	 & 14.68	& 19.32	& 27.66 \\
LLava-Next-Llama3-8B~\cite{llavanext}     & 20.01	 & 28.69	& 15.01	& 26.38 \\
mPLUG-Owl (v2)-9.2B~\cite{mplug}    & \textbf{24.31}	& 26.74	&\textbf{20.51}	&\textbf{30.97}\\
Blip-2-12B~\cite{blip2} &  17.75	&26.00	&22.00	&37.00  \\
InstructBLIP-12B~\cite{instructblip} & 10.23	 &00.46	&17.19	&19.51 \\
OpenCLIP-CoCa-13B ~\cite{coca}   &18.79	&21.59	&12.02	&24.40\\
MiniGPT4-Vicuna-13B~\cite{minigpt}    & 12.79	&16.21	&17.10	&24.51 \\
CogVLM v2 (llama3)-17B~\cite{cogvlm}    &21.86	&30.31	&18.63	&28.67 \\ 
LLaVA-Next-Qwen110B~\cite{llavanext}       & 19.73	& 27.18	& 14.96	& 26.61 \\
GPT-4o                   &21.86	&\textbf{32.56}	&18.56	&28.37 \\
GPT-4V                   & 17.36	 &11.24	&19.47	&26.75 \\ \hline \hline
\end{tabular} %
}
\caption{\textbf{Zero-shot Evaluation on Imaginary Image Captioning.} The best results are highlighted in bold. The low scores on the metrics indicate the baseline models struggle to describe imaginary images.}
\label{tab:ugc_result}
\end{minipage}
\end{table}

%\footnote{https://platform.openai.com/docs/guides/vision}
%\footnote{https://platform.openai.com/docs/guides/vision} 

==> tables/cross_two_row.tex <==
\begin{table}[t]
% \small
\captionsetup{skip=5pt}
\centering
% \fontsize{8}{9}
\selectfont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.4}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccccccccc}
\hline 
\hline
\multicolumn{1}{l}{} & \multicolumn{10}{c}{\textbf{Text Retrieval}} \\ \hline

\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Flickr30K(1K)} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}MS-COCO-Full\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}MS-COCO(1K)\end{tabular}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}JourneyBench(1K)\\ w/o distractors\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}JourneyBench(1K)\\ w/ distractors\end{tabular}}} \\ \cline{2-12}

 & R@1 & \multicolumn{1}{c|}{R@5} & R@1 & \multicolumn{1}{c|}{R@5} & R@1 & \multicolumn{1}{c|}{R@5} & R@1 & \multicolumn{1}{c|}{R@5} & R@1 & R@5 \\ \hline

ALBEF-210M~\cite{albef} & 88.50 & \multicolumn{1}{c|}{98.50} & 73.96 & \multicolumn{1}{c|}{91.80} & 89.10 & \multicolumn{1}{c|}{98.30} & 72.30 & \multicolumn{1}{c|}{86.10} & 65.36 & 83.75 \\ 

CLIP-430M~\cite{clip} & 85.30 & \multicolumn{1}{c|}{97.90} & 58.40 & \multicolumn{1}{c|}{81.50} & 75.60 & \multicolumn{1}{c|}{93.20} & 70.60 & \multicolumn{1}{c|}{85.70} & 60.80 & 83.30 \\

X2\_VLM-Large-590M~\cite{x2vlm} & 98.80 & \multicolumn{1}{c|}{100} & 84.40 & \multicolumn{1}{c|}{96.50} & 93.60  & \multicolumn{1}{c|}{99.50} & 78.54 & \multicolumn{1}{c|}{92.78}  & 64.97 & \textbf{90.47}  \\

BEiT3-674M~\cite{beit3} & 89.50 & \multicolumn{1}{c|}{98.80} & 64.00 & \multicolumn{1}{c|}{ 86.60} & 81.10  & \multicolumn{1}{c|}{96.60} & 81.10 & \multicolumn{1}{c|}{\textbf{96.60}}  & 65.90 & 86.10 \\


BLIP2-12B~\cite{blip2} & 92.80 & \multicolumn{1}{c|}{99.90} & 80.10 & \multicolumn{1}{c|}{94.80} & 91.30 & \multicolumn{1}{c|}{99.10} & \textbf{81.29} &\multicolumn{1}{c|}{95.17}  & 63.78 & 87.76  \\

OpenCLIP-CoCa-13B~\cite{coca} & 92.50 & \multicolumn{1}{c|}{99.50} & 66.30 & \multicolumn{1}{c|}{86.20} & 75.89  & \multicolumn{1}{c|}{93.63} & 70.43 & \multicolumn{1}{c|}{85.41}  & 60.04 & 83.32\\ 

InternVL-C-13B~\cite{Internvl} & 94.70 & \multicolumn{1}{c|}{99.60} & 74.90 & \multicolumn{1}{c|}{91.30} & 85.34 & \multicolumn{1}{c|}{96.86} & 78.22 & \multicolumn{1}{c|}{89.21}  & \textbf{67.73} & 86.41  \\

InternVL-G-14B~\cite{Internvl} & 95.70 & \multicolumn{1}{c|}{99.70} & 74.90 & \multicolumn{1}{c|}{91.30} & 87.58  & \multicolumn{1}{c|}{97.64} & 78.52 & \multicolumn{1}{c|}{89.81}  & 67.53 & 86.51 \\ \hline 


\multicolumn{1}{l}{} & \multicolumn{10}{c}{\textbf{Image Retrieval}} \\ \hline

ALBEF-210M~\cite{albef} & 75.90 & \multicolumn{1}{c|}{92.60} & 54.00 & \multicolumn{1}{c|}{78.99} & 72.28 & \multicolumn{1}{c|}{94.18} & 66.12 & \multicolumn{1}{c|}{88.65}  &50.02 & 75.46\\

CLIP-430M~\cite{clip} & 64.90 & \multicolumn{1}{c|}{87.20} & 37.80 & \multicolumn{1}{c|}{62.40} & 54.50 & \multicolumn{1}{c|}{81.80} & 66.80 & \multicolumn{1}{c|}{88.80} & 51.20 & 76.50 \\

X2\_VLM-Large-590M~\cite{x2vlm} & 91.80 & \multicolumn{1}{c|}{98.60} & 67.70 & \multicolumn{1}{c|}{87.50} & 83.32 & \multicolumn{1}{c|}{96.86} & 75.04 &\multicolumn{1}{c|}{93.16} & 61.02 & 85.00 \\

BEiT3-674M~\cite{beit3} & 75.94 & \multicolumn{1}{c|}{93.34} & 48.90 & \multicolumn{1}{c|}{73.20} & 66.40  & \multicolumn{1}{c|}{89.50} & 68.00 & \multicolumn{1}{c|}{90.30} & 56.20 & 79.90 \\

BLIP2-12B~\cite{blip2} & 89.70 & \multicolumn{1}{c|}{98.10} & 63.00 & \multicolumn{1}{c|}{84.20} & 78.78  & \multicolumn{1}{c|}{94.92} & 75.77 & \multicolumn{1}{c|}{91.66}  & 59.97 & 82.48 \\

OpenCLIP-CoCa-13B~\cite{coca} & 80.40 & \multicolumn{1}{c|}{95.70} & 51.20 & \multicolumn{1}{c|}{74.20} & 59.30 & \multicolumn{1}{c|}{85.51} & 65.83 & \multicolumn{1}{c|}{86.66} & 48.70 & 72.56 &  \\

InternVL-C-13B~\cite{Internvl} & 81.70 & \multicolumn{1}{c|}{96.00} & 54.10 & \multicolumn{1}{c|}{77.30} & 71.43 & \multicolumn{1}{c|}{91.50} & 75.84 & \multicolumn{1}{c|}{93.34}  & 62.29 & 83.44 \\

InternVL-G-14B~\cite{Internvl} & 85.00 & \multicolumn{1}{c|}{97.00} & 58.60 & \multicolumn{1}{c|}{81.30} & 75.64 & \multicolumn{1}{c|}{93.77} & \textbf{76.80} & \multicolumn{1}{c|}{\textbf{93.80}} & \textbf{63.71} & \textbf{84.84}  \\  \hline \hline
\end{tabular}%
}
\caption{\textbf{Zero-shot Evaluation of Cross-modal Retrieval.} The best results are highlighted in bold. The performance of baseline models on JourneyBench without distractors is comparable to that of existing cross-modal retrieval tasks of similar scale, indicating their generalizability to generated images. However, there is a notable decline in performance when distractors are added, highlighting the critical role of sample-specific distractors in enhancing the challenge of the retrieval tasks.}
\label{tab:crossmodal-retrieval-result}
\end{table}


==> tables/imaginary-image-captioning-result-table.tex <==
\begin{table}[ht!]\small
\captionsetup{skip=5pt}
\centering
\fontsize{8}{9}\selectfont
\setlength{\tabcolsep}{3pt}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|lcl} \hline \hline
Model                    & BLEU1-4         & CIDEr        & METEOR       & Rouge        \\ \hline
MiniGPT4-LLama2-7B~\cite{minigpt}      & 0.20	& 0.21 &0.18	&0.29 \\
mPLUG-Owl-7.2B~\cite{mplug}       & 0.20	 & 0.15	& 0.19	& 0.28 \\
LLava-Next-Llama3-8B~\cite{llavanext}     &0.20	 &0.29	&0.15	&0.26 \\
mPLUG-Owl (v2)-9.2B~\cite{mplug}    & \textbf{0.24}	&0.27	&\textbf{0.21}	&\textbf{0.31 }\\
Blip-2-12B~\cite{blip2}     &          &      &         &                 \\
InstructBLIP-12B~\cite{instructblip} & 0.10	 &0.00	&0.17	&0.20 \\
OpenCLIP-CoCa-13B ~\cite{coca}   &0.19	&0.22	&0.12	&0.24\\
MiniGPT4-Vicuna-13B~\cite{minigpt}    & 0.13	&0.16	&0.17	&0.25 \\
CogVLM v2 (llama3)-17B~\cite{cogvlm}    &0.22	&0.30	&0.19	&0.29 \\ 
LLaVA-Next-Qwen110B~\cite{llavanext}       & 0.20	&0.27	&0.15	&0.27 \\
GPT-4o                   &0.22	&\textbf{0.33}	&0.19	&0.28 \\
GPT-4V                   & 0.17	 &0.11	&0.19	&0.27 \\

\hline \hline
\end{tabular} %
%}
\caption{Zero-shot Evaluation on Unusual Caption Generation in our JourneyBench unusual caption generation dataset. The best results are highlighted in bold.}
\label{tab:ugc_result}
\end{table}


==> tables/multi-image_vqa-result-table.tex <==
%{\begin{table}[ht]
%    \centering
%   \begin{tabular}{|c|c|c|c|c|c|} \hline
%    \multirow{2}{*}{Model} &\multicolumn{4}{|c|}{Ours} &\multirow{2}{*}{Mantis-Eval} \\ \cline{2-5}
%              &All &MCOT &External Knowledge &Cause-and-Effect & \\ \hline
%    VILA-8B     &  7.26 &8.66 &8.65 &   &51.15 \\ %\hline
%    Idefices2-8B     & 7.82 &7.82   &10.57 &65.03 &48.85 \\ %\hline
%    Mantis-Idefics2-8B &3.91 &4.54 &2.88 &49.02 &57.14 \\ %\hline
%    Mantis-SigLIP-8B &5.59 & &3.41  &55.88 &59.45 \\ %\hline
%    GPT-4V & &32.4 &32.2 &77.06 &62.67 \\ %\hline
%    GPT-4o &40.22 &61.2 &29.61 &83.33 & \\ \hline
%    \end{tabular}
%    \caption{Zero-shot Evaluation on Multi-Image MCOT dataset}
%    \label{tab:multi-image mcot}
%\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht!]\small
\captionsetup{skip=5pt}
\centering
\fontsize{8}{9}\selectfont
\setlength{\tabcolsep}{3pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|l|l|m{1 cm}|m{1 cm}|c|l}
\hline \hline
\multirow{3}{*}{Model} & \multicolumn{5}{c|}{Multi-Image VQA} & \multirow{3}{*}{\makecell{Mantis\\Eval}} \\ \cline{2-6}
   &   \multirow{2}{*}{All} &  \multicolumn{3}{c|}{MMCOT} & \multirow{2}{*}{\makecell{Cause \\and \\ Effect}} &  \\ \cline{3-5}
   &   & \multicolumn{1}{l|}{All} &\multicolumn{1}{l|}{\makecell{Arithmetic \\ Reasoning}} & \multicolumn{1}{l|}{\makecell{External\\Knowledge}} &   & \\ \hline
VILA-8B~\cite{vila}            &       & 6.14  & 3.73  & 8.65  & 53.92 & 51.15 \\
Idefics2-8B~\cite{idefics2}        & 27.82 & 6.61  & 2.81  & 10.57 & 65.03 & 48.85 \\
Mantis-Idefics2-8B~\cite{mantis} & 19.90 & 3.30  & 3.71  & 2.88  & 49.02 & 57.14 \\
Mantis-SigLIP-8B~\cite{mantis}   & 23.29 & 4.72  & 5.98  & 3.41  & 55.88 & 59.45 \\
GPT-4V~\footnote{https://platform.openai.com/docs/guides/vision}              & 48.70 & 32.54 & 32.88 & 32.2  &77.06 & \textbf{62.67} \\
GPT-4o~\footnote{https://platform.openai.com/docs/guides/vision}             & \textbf{56.39} & \textbf{41.03} & \textbf{52.04} & \textbf{29.61 }& \textbf{83.33} &     \\ \hline \hline
\end{tabular}

\caption{Zero-shot evaluation on our JourneyBench's Multi-Image MCOT and Multi-Image VQA datasets. The best results are highlighted in bold.}
    \label{tab:multi-image mcot}
\end{table}

% 
